Stochastic Network Utility Maximization with Unknown Utilities: Multi-Armed Bandits Approach

In this paper, we study a novel Stochastic Network Utility Maximization (NUM) problem where the utilities of agents are unknown. The utility of each agent depends on the amount of resource it receives from a network operator/controller. The operator desires to do a resource allocation that maximizes the expected total utility of the network. We consider threshold type utility functions where each agent gets non-zero utility if the amount of resource it receives is higher than a certain threshold. Otherwise, its utility is zero (hard real-time). We pose this NUM setup with unknown utilities as a regret minimization problem. Our goal is to identify a policy that performs as `good' as an oracle policy that knows the utilities of agents. We model this problem setting as a bandit setting where feedback obtained in each round depends on the resource allocated to the agents. We propose algorithms for this novel setting using ideas from Multiple-Play Multi-Armed Bandits and Combinatorial Semi-Bandits. We show that the proposed algorithm is optimal when all agents have the same utility. We validate the performance guarantees of our proposed algorithms through numerical experiments.

==> discussion.tex <==
%!TEX root =  main.tex

\noindent
\textbf{Issue with only two thresholds:}

~\\
\textbf{$\gamma$ issues?}
	



==> experiment_results.tex <==
%!TEX root =  main.tex

%\begin{figure}[H]
%	\begin{minipage}[b]{0.50\textwidth}
%		\captionsetup{justification=centering}
%		\captionsetup{font=scriptsize, labelfont=bf}
%		\includegraphics[width=0.48\linewidth]{results/berSameThetaC_10000_50_20.png}
%		\includegraphics[width=0.48\linewidth]{results/berSameThetaT_10000_50_20.png}
%		\caption{Arms are having Bernoulli distributed reward and same threshold.}
%		\label{fig:BerSameTheta}
%	\end{minipage}
%	\begin{minipage}[b]{0.50\textwidth}
%		\captionsetup{justification=centering}
%		\captionsetup{font=scriptsize, labelfont=bf}
%		\includegraphics[width=0.48\linewidth]{results/uniSameThetaC_10000_50_20.png}
%		\includegraphics[width=0.48\linewidth]{results/uniSameThetaT_10000_50_20.png}
%		\caption{Arms are having Uniform distributed reward and same threshold.}
%		\label{fig:UnifSameTheta}
%	\end{minipage}
%\end{figure}
%
%\begin{figure}[H]
%	\begin{minipage}[b]{0.50\textwidth}
%		\captionsetup{justification=centering}
%		\captionsetup{font=scriptsize, labelfont=bf}
%		\includegraphics[width=0.48\linewidth]{results/berDiffThetaC__10000_5_20.png}
%		\includegraphics[width=0.48\linewidth]{results/berDiffThetaC__10000_10_20.png}
%		\caption{Arms are having Bernoulli distributed reward and different threshold.}
%		\label{fig:BerDiffTheta}
%	\end{minipage}
%	\begin{minipage}[b]{0.50\textwidth}
%		\captionsetup{justification=centering}
%		\captionsetup{font=scriptsize, labelfont=bf}
%		\includegraphics[width=0.48\linewidth]{results/uniDiffThetaC_10000_5_20.png}
%		\includegraphics[width=0.48\linewidth]{results/uniDiffThetaC_10000_10_20.png}
%		\caption{Arms are having Uniform distributed reward and different threshold.}
%		\label{fig:UnifDiffTheta}
%	\end{minipage}
%\end{figure}
\begin{figure*}[!ht]
	\centering
	\begin{subfigure}[b]{0.245\textwidth}
		\includegraphics[width=\linewidth]{results/berSameThetaC_10000_50_50.png}
		\caption{\footnotesize Bernoulli Distributed Reward}
		\label{fig:BerSameThetaC}
	\end{subfigure}
	\begin{subfigure}[b]{0.245\textwidth}
		\includegraphics[width=\linewidth]{results/uniSameThetaC_10000_50_50.png}
		\caption{\footnotesize Uniform Distributed Reward}
		\label{fig:UniSameThetaC}	
	\end{subfigure}
	\begin{subfigure}[b]{0.245\textwidth}
		\includegraphics[width=\linewidth]{results/berSameThetaT_10000_50_50.png}
		\caption{\footnotesize Bernoulli Distributed Reward}
		\label{fig:BerSameThetaT}
	\end{subfigure}
	\begin{subfigure}[b]{0.245\textwidth}
		\includegraphics[width=\linewidth]{results/uniSameThetaT_10000_50_50.png}
		\caption{\footnotesize Uniform Distributed Reward}
		\label{fig:UniSameThetaT}
	\end{subfigure}
	%	\captionsetup{justification=centering}
	\caption{Cumulative Regret of ONUM-S with Bernoulli and Uniform distributed rewards for same threshold.}
	\label{fig:SameTheta}
\end{figure*}

\begin{figure*}[!ht]
	\centering
	\begin{subfigure}[b]{0.245\textwidth}
		\includegraphics[width=\linewidth]{results/berDiffThetaC_10000_5_50.png}
		\caption{\footnotesize Bernoulli Distributed Reward}
		\label{fig:BerDiffTheta2}
	\end{subfigure}
	\begin{subfigure}[b]{0.245\textwidth}
		\includegraphics[width=\linewidth]{results/uniDiffThetaC_10000_5_200.png}
		\caption{\footnotesize Uniform Distributed Reward}
		\label{fig:UniDiffTheta2}
	\end{subfigure}
	\begin{subfigure}[b]{0.245\textwidth}
		\includegraphics[width=\linewidth]{results/berDiffThetaC_10000_10_50.png}
		\caption{\footnotesize Bernoulli Distributed Reward}
		\label{fig:BerDiffTheta3}
	\end{subfigure}	
	\begin{subfigure}[b]{0.245\textwidth}
		\includegraphics[width=\linewidth]{results/uniDiffThetaC_10000_10_200.png}
		\caption{\footnotesize Uniform Distributed Reward}
		\label{fig:UniDiffTheta3}
	\end{subfigure}
	%	\captionsetup{justification=centering}
	\caption{Cumulative Regret of ONUM-D with Bernoulli and Uniform distributed rewards for different threshold.}
	\label{fig:DiffTheta}
\end{figure*}
